Measure Transport with Kernel Stein Discrepancy

Measure transport underpins several recent algorithms for posterior approximation in the Bayesian context, wherein a transport map is sought to minimise the Kullback--Leibler divergence (KLD) from the posterior to the approximation. The KLD is a strong mode of convergence, requiring absolute continuity of measures and placing restrictions on which transport maps can be permitted. Here we propose to minimise a kernel Stein discrepancy (KSD) instead, requiring only that the set of transport maps is dense in an $L^2$ sense and demonstrating how this condition can be validated. The consistency of the associated posterior approximation is established and empirical results suggest that KSD is competitive and more flexible alternative to KLD for measure transport.

==> Measure Transport with Kernel Stein Discrepancy/abstract.tex <==
Measure transport underpins several recent algorithms for posterior approximation in the Bayesian context, wherein a transport map is sought to minimise the Kullback--Leibler divergence (KLD) from the posterior to the approximation. 
The KLD is a strong mode of convergence, requiring absolute continuity of measures and placing restrictions on which transport maps can be permitted.
Here we propose to minimise a kernel Stein discrepancy (KSD) instead, requiring only that the set of transport maps is dense in an $L^2$ sense and demonstrating how this condition can be validated.
The consistency of the associated posterior approximation is established and empirical results suggest that KSD is competitive and more flexible alternative to KLD for measure transport.

==> Measure Transport with Kernel Stein Discrepancy/body.tex <==


\section{Introduction}
\label{sec:introduction}

A popular and constructive approach to approximation of complicated distributions is to learn a transformation from a simpler reference distribution.
Within machine learning, neural networks are often used to provide flexible families of transformations which can be optimised by stochastic gradient descent on a suitable objective, with \emph{variational autoencoders} \citep{kingma2013,rezende2014stochastic}, \emph{generative adversarial networks} \citep{goodfellow2014generative}, \emph{generative moment matching networks} \citep{li2015generative,dziugaite2015training} and \emph{normalizing flows}
\citep{rezende2015variational, kingma, dinh2016density, papamakarios2019normalizing, Kobyzev_2020} all fitting in this framework.
The principal application for such generative models is \emph{distribution estimation};
samples are provided from the target distribution and the task is to fit a distribution to these samples. Parallel developments within applied mathematics view the transformation as a \emph{transport map} performing \emph{measure transport} \citep{Marzouk_2016, parno2018transport}. The principal application for measure transport is \emph{posterior approximation}; an un-normalised density function defines the complicated distribution and the task is to approximate it.
In this paper we study posterior approximation, noting that the flexible transformations developed in the machine learning literature can also be applied to this task.

Measure transport provides a powerful computational tool for Bayesian inference in settings that can be challenging for standard approaches, such as Markov chain Monte Carlo (MCMC) or mean field variational inference.
For example, even sophisticated MCMC methods can fail when a posterior is concentrated around a sub-manifold of the parameter space \citep{livingstone2019robustness, au2020manifold}, while it can be relatively straight-forward to define a transport map whose image is the sub-manifold \citep{parno2018transport, brehmer2020flows}.
Likewise, mean field variational inference methods can perform poorly in this context, since independence assumptions can be strongly violated \citep{blei2017variational}.

Let $\mathcal{Y}$ be a measurable space equipped with a probability measure $P$, representing the posterior to be approximated.
The task that we consider in this paper is to elicit a second measurable space $\mathcal{X}$, equipped with a probability measure $Q$, and a measurable function $T : \mathcal{X} \rightarrow \mathcal{Y}$, such that the push-forward $T_\# Q$ (i.e.~the measure produced by applying $T$ to samples from $Q$) approximates $P$, in a sense to be specified. It is further desired that $Q$ should be a ``simple'' distribution that is easily sampled. In contrast to the literature on normalising flows, it is \emph{not} stipulated that $T$ should be a bijection, since we wish to allow for situations where $\mathcal{X}$ and $\mathcal{Y}$ have different cardinalities or where $P$ is supported on a sub-manifold.

A natural starting point is a notion of \emph{discrepancy} $\mathcal{D}(P_1,P_2)$ between two probability measures, $P_1$ and $P_2$, on $\mathcal{Y}$, with the property that $\mathcal{D}(P_1,P_2) = 0$ if and only if $P_1$ and $P_2$ are equal. Then one selects a measurable space $\mathcal{X}$ and associated probability measure $Q$ and seeks a solution to
\begin{equation} \label{eq:minproblem1}
\argmin_{T \in \mathcal{T}} \mathcal{D}(P,T_\# Q),
\end{equation}
over a suitable set $\mathcal{T}$ of measurable functions from $\mathcal{X}$ to $\mathcal{Y}$. A popular choice of $\mathcal{D}$ is the Kullback-Leibler divergence (KLD), giving rise to \emph{variational inference} \citep{blei2017variational}, but other discrepancies can be considered \citep{ranganath2016operator}. The problem in \eqref{eq:minproblem1} can be augmented to include also the selection of $\mathcal{X}$ and $Q$, if desired.

The solution of \eqref{eq:minproblem1} provides an approximation to $P$ whose quality will depend on the set $\mathcal{T}$ and the discrepancy $\mathcal{D}$. This motivates us to consider the choice of $\mathcal{T}$ and $\mathcal{D}$, taking into account considerations that go beyond computational tractability. For example, a desirable property would be that, for a sequence of probability measures $(P_n)_{n\in\mathbb{N}}$, if $\mathcal{D}(P,P_n) \rightarrow 0$ then $P_n \rightarrow P$ in some suitable sense. For $\mathcal{D} = \mathcal{D}_{\text{KL}}$, the KLD\footnote{We use the notation $\mathcal{D}_{\text{KL}}(P,Q) \coloneqq \text{KL}(Q||P)$.}, it holds that $\mathcal{D}_{\text{KL}}(P,P_n) \rightarrow 0$ implies $P_n$ converges to $P$ in \emph{total variation}, from Pinsker's inequality \citep{tsybakov2008nonparametric}. This is a strong mode of convergence, requiring absolute continuity of measures that may be difficult to ensure when the posterior is concentrated near to a sub-manifold. Accordingly, the use of KLD for measure transport places strong and potentially impractical restrictions on which maps $T$ are permitted \citep[e.g.][required that $T$ is a diffeomorphism with $\text{det}\nabla T > 0$ on $\mathcal{X}$]{Marzouk_2016,parno2018transport}. This motivates us in this paper to consider the use of an alternative discrepancy $\mathcal{D}$, corresponding to a weaker mode of convergence, for posterior approximation using measure transport. The advantage of discrepancy measures inducing weaker modes of convergence has also motivated recent developments in generative adversarial networks \citep{arjovsky2017wasserstein}.


Our contributions are as follows:

\begin{itemize} 
	\item We propose kernel Stein discrepancy (KSD) as an alternative to KLD for posterior approximation using measure transport, showing that KSD renders \eqref{eq:minproblem1} tractable for standard stochastic optimisation methods (\Cref{prop: gradients}).
	\item Using properties of KSD we are able to establish consistency under explicit and verifiable assumptions on $P$, $Q$ and $\mathcal{T}$ (\Cref{theorem: convergence theorem}). 
	\item Our theoretical assumptions are weak -- we do not even require $T$ to be a bijection -- and are verified for a particular class of neural network (\Cref{prop: ReLU DNN}).
	In particular, we do not require $Q$ and $P$ to be defined on the same space, allowing quite flexible mappings $T$ to be constructed.
	\item Empirical results support KSD as a competitive alternative to KLD for measure transport.
\end{itemize}

Earlier work on this topic appears limited to \cite{hu2018stein}, who trained a neural network with KSD.
Here we consider general transport maps and we establish consistency of the method, which these earlier authors did not.
We note also that gradient flows provide an alternative (implicit) approach to measure transport \citep{liu2016stein}.

\paragraph{Outline:}
The remainder of the paper is structure as follows: \Cref{sec:methodology} introduces measure transport using KSD, \Cref{sec: theory} contains theoretical analysis for this new method, \Cref{sec:experiments} presents a detailed empirical assessment and \Cref{sec: discuss} contains a discussion of our main findings. 

\section{Methods} \label{sec:methodology}

This section introduces measure transport using KSD.
In \Cref{subsec: measure transport} and \Cref{subsec: RKHS} we recall mathematical definitions from measure transport and Hilbert spaces, respectively; in \Cref{subsec: KSD} we recall the definition and properties of KSD; in \Cref{subsec: methodology} we formally define our proposed method, and in \Cref{subsec: transport maps section} we present some parametric families $\mathcal{T}$ that can be employed.

\paragraph{Notation:}
The set of probability measures on a measurable space $\mathcal{X}$ is denoted $\mathcal{P}(\mathcal{X})$ and a point mass at $x \in \mathcal{X}$ is denoted $\delta(x) \in \mathcal{P}(\mathcal{X})$. For $P \in \mathcal{P}(\mathcal{X})$ let $L^q(P) := \{f : \mathcal{X} \rightarrow \mathbb{R} : \int f^q \mathrm{d}P < \infty\}$. For $P \in \mathcal{P}(\mathbb{R}^d)$ and $(P_n)_{n \in \mathbb{N}} \subset \mathcal{P}(\mathbb{R}^d)$, let $P_n \Rightarrow P$ denote weak convergence of the sequence of measures $(P_n)_{n \in \mathbb{N}}$ to $P$. The Euclidean norm on $\mathbb{R}^n$ is denoted $\|\cdot\|$. Partial derivatives are denoted $\partial_{x}$. For a function $f:\mathbb{R}^n\rightarrow\mathbb{R}$ the gradient is defined as $[\nabla f]_{i} = \partial_{x_i} f$. For a function $f = (f_1,\ldots,f_m) : \mathbb{R}^n \rightarrow \mathbb{R}^m$, the divergence is defined as $\nabla \cdot f = \sum_{i=1}^n \partial_{x_i} f_i$.

Our main results in this paper concern the Euclidean space $\mathbb{R}^d$, but in some parts of the paper, such as \Cref{subsec: measure transport}, it is possible to state definitions at a greater level of generality at no additional effort - in such situations we do so.


\subsection{Measure Transport} \label{subsec: measure transport}

A \emph{Borel space} $\mathcal{X}$ is a topological space equipped with its Borel $\sigma$-algebra, denoted $\Sigma_\mathcal{X}$.
Throughout this paper we restrict attention to Borel spaces $\mathcal{X}$ and $\mathcal{Y}$. Let $Q \in \mathcal{P}(\mathcal{X})$ and $P \in \mathcal{P}(\mathcal{Y})$. In the parlance of measure transport,  $Q$ is the \emph{reference} and $P$ the \emph{target}. Let $T : \mathcal{X} \rightarrow \mathcal{Y}$ be a measurable function and define the \emph{pushforward} of $Q$ through $T$ as the probability measure $T_\# Q \in \mathcal{P}(\mathcal{Y})$ that assigns mass $(T_\# Q)(A) = Q(T^{-1}(A))$ to each $A\in\Sigma_\mathcal{Y}$. Here $T^{-1}(A) = \{x \in \mathcal{X} : T(x) \in A\}$ denotes the pre-image of $A$ under $T$.
Such a function $T$ is called a \emph{transport map} from $Q$ to $P$ if $T_\# Q = P$. 

Faced with a complicated distribution $P$, if one can express $P$ using a transport map $T$ and a distribution $Q$ that can be sampled, then samples from $P$ can be generated by applying $T$ to samples from $Q$. This idea underpins elementary methods for numerical simulation of random variables \citep{devroye2013}. However, in posterior approximation it will not typically be straightforward to identify a transport map and at best one can seek an \emph{approximate} transport map, for which $T_\# Q$ approximates $P$ in some sense to be specified. In this paper we seek approximations in the sense of KSD, which is formally introduced in \Cref{subsec: KSD} and requires concepts in \Cref{subsec: RKHS}, next.


\subsection{Hilbert Spaces} \label{subsec: RKHS}

A Hilbert space $\mathcal{H}$ is a complete inner product space; in this paper we use subscripts, such as $\langle \cdot , \cdot \rangle_{\mathcal{H}}$, to denote the associated inner product. Given two Hilbert spaces $\mathcal{G}$, $\mathcal{H}$, the \emph{Cartesian product} $\mathcal{G} \times \mathcal{H}$ is again a Hilbert space equipped with the inner product $\langle (g_1,h_1), (g_2,h_2) \rangle_{\mathcal{G} \times \mathcal{H}} := \langle g_1, g_2 \rangle_{\mathcal{G}} + \langle h_1, h_2 \rangle_{\mathcal{H}}$.
In what follows we let $\mathcal{B}(\mathcal{H}) := \{ h \in \mathcal{H} : \langle h , h \rangle_{\mathcal{H}} \leq 1 \}$ denote the unit ball in a Hilbert space $\mathcal{H}$.

From the Moore--Aronszajn theorem \citep{aronszajn1950theory}, any symmetric positive definite function $k : \mathcal{Y} \times \mathcal{Y} \rightarrow \mathbb{R}$ defines a unique \emph{reproducing kernel Hilbert space} of real-valued functions on $\mathcal{Y}$, denoted $\mathcal{H}_k$ and with inner-product denoted $\langle \cdot , \cdot \rangle_{\mathcal{H}_k}$. Indeed, $\mathcal{H}_k$ is a Hilbert space characterised by the properties (i) $k(\cdot,y) \in \mathcal{H}_k$ for all $y \in \mathcal{Y}$, (ii) $\langle h , k(\cdot,y) \rangle_{\mathcal{H}_k} = h(y)$ for all $h \in \mathcal{H}_k$, $y \in \mathcal{Y}$. Reproducing kernels are central to KSD, as described next.




\subsection{Kernel Stein Discrepancy} \label{subsec: KSD}

Stein discrepancies were introduced in \cite{gorham2015measuring} to provide a notion of discrepancy that is computable in the Bayesian statistical context. In this paper we focus on so-called \emph{kernel Stein discrepancy} \cite[KSD;][]{liu2016kernelized,chwialkowski2016kernel,gorham2017measuring} since this has lower computational overhead compared to the original proposal of \cite{gorham2015measuring}.


The construction of KSD relies on Stein's method \citep{stein1972} where, for a possibly complicated probability measure $P \in \mathcal{P}(\mathcal{Y})$ of interest, one identifies a \emph{Stein set} $\mathcal{F}$ and a \emph{Stein operator} $\mathcal{A}_P$, such that $\mathcal{A}_P$ acts on elements $f \in \mathcal{F}$ to return functions $\mathcal{A}_P f : \mathcal{Y} \rightarrow \mathbb{R}$ with the property that
\begin{equation}
P' = P \quad \text{iff} \quad \E_{Y \sim P'}[(\mathcal{A}_P f)(Y)] = 0 \; \forall f\in\mathcal{F} \label{eq: stein identity}
\end{equation}
for all $P' \in \mathcal{P}(\mathcal{Y})$.
A \emph{Stein discrepancy} uses the extent to which \eqref{eq: stein identity} is violated to quantify the discrepancy between $P'$ and $P$:
\begin{align*}
\mathcal{D}_{\text{S}}(P,P') := \sup_{f \in \mathcal{F}} |\E_{Y\sim P'}[(\mathcal{A}_P f)(Y)]|
\end{align*}
Note that $\mathcal{D}_{\text{S}}$ is not symmetric in its arguments.
For $\mathcal{Y} = \mathbb{R}^d$ and suitably regular $P$, which admits a positive and differentiable density function $p$, \cite{liu2016kernelized,chwialkowski2016kernel} showed that one may take $\mathcal{F}$ to be a set of smooth vector fields $f : \mathbb{R}^d \rightarrow \mathbb{R}^d$ and $\mathcal{A}_P$ to be a carefully chosen differential operator on $\mathbb{R}^d$. More precisely, and letting $s_p := \nabla \log p$, we have \Cref{theorem:gorham inverse multi quadric} below, which is due to \citet[][Theorem 7]{gorham2017measuring}:

\begin{definition}[\cite{Eberle_2015}]
	A probability measure $P \in \mathcal{P}(\mathbb{R}^d)$ is called \emph{distantly dissipative} if $\liminf_{r\rightarrow \infty} \kappa(r) > 0$, where
	\begin{equation*} 
	%\kappa(r) \coloneqq \inf_{\|x-y\| = r} - \frac{\langle s_p(x) -s_p(y),x-y\rangle}{\|x-y\|^2}.
	\textstyle \kappa(r) \coloneqq -r^{-2} \inf_{\|x-y\| = r} \langle s_p(x) -s_p(y),x-y\rangle. 
	\end{equation*}
\end{definition}

\begin{theorem}
	\label{theorem:gorham inverse multi quadric} Suppose that $P \in \mathcal{P}(\mathbb{R}^d)$ is distantly dissipative. 
	For some $c>0$, $\ell > 0$ and $\beta \in (-1,0)$, let
	\begin{eqnarray}
	\hspace{-5pt} \mathcal{F} := \textstyle \mathcal{B} \big( \prod_{i=1}^d \mathcal{H}_k \big), \quad k(x,y) := (c^2 + \|\frac{x-y}{\ell}\|^2)^\beta \label{eq: IMQ} \\
	\mathcal{A}_P f := f\cdot\nabla \log p + \nabla\cdot f  . \hspace{60pt}
	\end{eqnarray} 
	Then \eqref{eq: stein identity} holds.
	Moreover, if $\mathcal{D}_{\textsc{S}}(P,P_n)\rightarrow 0$, then $P_n \Rightarrow P$. 
\end{theorem}

The kernel $k$ appearing in \eqref{eq: IMQ} is called the \emph{inverse multi-quadric} kernel.
It is known that the elements of $\mathcal{H}_k$ are smooth functions, which justifies the application of the differential operator.
The last part of \Cref{theorem:gorham inverse multi quadric} clarifies why KSD is useful; convergence in KSD controls the standard notion of weak convergence of measures to $P$. 

KSD, in contrast to KLD, is well-defined when the approximating measure $P'$ and the target $P$ differ in their support.
Moreover, in some situations KSD can be exactly computed: from \citet[][Theorem 3.6]{liu2016kernelized} or equivalently \citet[][Theorem 2.1]{chwialkowski2016kernel},
\begin{align}
\mathcal{D}_{\text{S}}(P,P') & = \sqrt{ \E_{Y,Y' \sim P'}[u_p(Y,Y')] } \label{eq:KSD compute} \\
u_p(y,y') & := s_p(y)^\top k(y,y') s_p(y') + s_p(y)^\top \nabla_{y'} k(y,y') \nonumber \\
& \hspace{-5pt} + \nabla_y k(y,y')^\top s_p(y') + \nabla_y\cdot\nabla_{y'} k(y,y'). \label{eq: up formula}
\end{align}
It follows that KSD can be exactly computed whenever $P'$ has a finite support and $s_p$ can be evaluated on this support:
\begin{align} \textstyle
\mathcal{D}_{\text{S}}\left(P, \frac{1}{n} \sum_{i=1}^n \delta(y_i) \right) = \sqrt{\frac{1}{n^2} \sum_{i,j=1}^n u_p(y_i,y_j)} . \label{eq: KSD final}
\end{align}
Computation of \eqref{eq: KSD final} can proceed with $p$ available up to an unknown normalisation constant, facilitating application in the Bayesian context. Now we are in a position to present our proposed method.


\subsection{Measure Transport with KSD} \label{subsec: methodology}



Our proposed method for posterior approximation is simply stated at a high level; we attempt to solve \eqref{eq:minproblem1} with $\mathcal{D} = \mathcal{D}_{\text{S}}$ and over a set $\mathcal{T}$ of candidate functions $T^\theta : \mathcal{X} \rightarrow \mathcal{Y}$ indexed by a finite-dimensional parameter $\theta \in \Theta$. That is, we aim to solve
\begin{equation} \label{eq:minproblem2}
\argmin_{\theta \in \Theta} \mathcal{D}_{\text{S}}(P,T_\#^\theta Q).
\end{equation}
Discussion of the choice of $\mathcal{T}$ is deferred until \Cref{subsec: transport maps section}.
Compared to previous approaches to measure transport using KLD \citep{rezende2015variational,kingma,Marzouk_2016,parno2018transport}, KSD is arguably more computationally and theoretically tractable; the computational aspects will now be described.

The solution of \eqref{eq:minproblem2} is equivalent to minimisation of the function $F(\theta) := \mathcal{D}_{\text{S}}(P,T_\#^\theta Q)^2$ over $\theta \in \Theta$. In order to employ state-of-the-art algorithms for stochastic optimisation, an unbiased estimator for the gradient $\nabla_\theta F(\theta)$ is required. A naive starting point would be to differentiate the expression for the KSD of an empirical measure in \eqref{eq: KSD final}, however the resulting \emph{V-statistic} is biased. Under weak conditions, we establish instead the following unbiased estimator (a \emph{U-statistic}) for the gradient:

\begin{proposition} \label{prop: gradients}
	Let $\Theta \subseteq \mathbb{R}^p$ be an open set.
	Assume that $\forall \theta \in \Theta$
	\begin{enumerate}[leftmargin=25pt]
		\item[(A1)] $(x,x') \mapsto u_p(T^\theta(x),T^\theta(x'))$ is measurable;
		\item[(A2)] $\mathbb{E}_{X,X' \sim Q}\left[ |u_p(T^\theta(X),T^\theta(X'))|\right] < \infty$;
		\item[(A3)] $\mathbb{E}_{X,X' \sim Q}\left[ \|\nabla_{\theta} u_p(T^\theta(X),T^\theta(X'))\|\right] < \infty$;
	\end{enumerate}
	and that $\forall x,x' \in \mathcal{X}$, 
	\begin{enumerate}[leftmargin=25pt]
		\item[(A4)] $\theta \mapsto \nabla_\theta u_p(T^\theta(x),T^\theta(x'))$ is continuous.
	\end{enumerate}
	Then $\forall \theta \in \Theta$
	\begin{align*} 
	\nabla_\theta F(\theta)
	= \textstyle \E\Big[ \frac{1}{n(n-1)} \sum\limits_{i \neq j} \nabla_\theta u_p(T^\theta(x_i),T^\theta(x_j)) \Big] ,
	\end{align*}
	where the expectation is taken with respect to independent samples $x_1,\dots,x_n \sim Q$.
\end{proposition}
All proofs are contained in \Cref{sec: proofs}.
The assumptions on $u_p$ amount to assumptions on $T$, $p$ and $k$, by virtue of \eqref{eq: up formula}.
It is not difficult to find explicit assumptions on $T$, $p$ and $k$ that imply (A1-4), but these may be stronger than required and we prefer to present the most general result.


Armed with an unbiased estimator of the gradient, we can employ a stochastic optimisation approach, such as stochastic gradient descent \citep[SGD;][]{robbins1951} or adaptive moment estimation \citep[Adam;][]{kingma2014adam}. 
See \cite{kushner2003stochastic, ruder2016overview}.
For the results reported in the main text we used Adam, with $\theta$ initialised as described in \Cref{subsec: initialise}, but other choices were investigated (see \Cref{subsec: stochastic optimisation}).


\subsection{Parametric Transport Maps} \label{subsec: transport maps section}

In this section we describe some existing classes of transport map $T : \mathcal{X} \rightarrow \mathcal{Y}$ that are compatible with KSD measure transport. 
From \Cref{prop: gradients} we see that measure transport using KSD does not impose strong assumptions on the transport map.
Indeed, compared to KLD \citep{rezende2015variational,kingma,Marzouk_2016,parno2018transport} we do not require that $T$ is a diffeomorphism ($T$ need not even be continuous, nor a bijection), making our framework considerably more general.
This additional flexibility may allow measure to be transported more efficiently, using simpler maps.
That being said, if one wishes to compute the density of $T_\# Q$ (in addition to sampling from $T_\# Q$), then a diffeomorphism, along with the usual change-of-variables formula, should be used.


\paragraph{Triangular Maps:}
\cite{rosenblatt1952remarks} and \cite{knothe1957contributions} observed that, for $P,Q \in \mathcal{P}(\mathbb{R}^d)$ admitting densities, a transport map $T:\mathbb{R}^d\rightarrow\mathbb{R}^d$ can without loss of generality be sought in the \emph{triangular form}
\begin{equation} \label{eq:lowertriangular}
T(x) = (T_1(x_1), T_2(x_1,x_2), \dots, T_d(x_1,\ldots,x_d) ),
\end{equation}
where each $T_i:\mathbb{R}^i \rightarrow \mathbb{R}$ and $x = (x_1,\ldots,x_d)$ \citep[][Lemma 2.1]{bogachev2005triangular}. The triangular form was used in \cite{Marzouk_2016,parno2018transport}, since the Jacobian determinant, that is required when using KLD (but not KSD), can exploit the fact that $\nabla T$ is triangular to maintain linear complexity in $d$. 

\paragraph{Maps from Measure Transport:}
In the context of a triangular map $T = (T_1,\ldots,T_d)$, \cite{Marzouk_2016} and \cite{parno2018transport} considered several parametric models for the components $T_i$, including polynomials, radial basis functions and monotone parameterisations of the form
\begin{align*}
T_i(x_1,\ldots,x_i) & = f_i(x_1,\ldots,x_{i-1}) \\
& \qquad + \textstyle \int_0^{x_i} \exp(g_i(x_1,\ldots,x_{i-1},y))\,\mathrm{d}y,
\end{align*}
for functions $f_i:\mathbb{R}^{i-1}\rightarrow\mathbb{R}$ and $g_i:\mathbb{R}^i\rightarrow\mathbb{R}$. %(for $i=1$, $f_i$ is a constant). 
The monotone parameterisation ensures that $\text{det}\nabla T > 0$ on $\mathbb{R}^d$, which facilitates computation of the density of $T_\#P$, as required for KLD\footnote{For polynomials and radial basis functions, these authors only enforced $\text{det}\nabla T > 0$ locally, introducing an additional approximation error in evaluation of KLD; such issues do not arise with KSD.}.


\paragraph{Maps from Normalising Flows:}
The principal application of normalising flows is density estimation \citep{papamakarios2019normalizing,Kobyzev_2020}, but the parametric families of transport map used in this literature can also be used for posterior approximation \citep{rezende2015variational}. A normalising flow is required to be a diffeomorphism $T : \mathbb{R}^d \rightarrow \mathbb{R}^d$ with the property that the density of $T_\#Q$ can be computed. A popular choice that exploits the triangular form \eqref{eq:lowertriangular} is an \textit{autoregressive flow} $T_i(x) = \tau(c_i(x_1,\ldots,x_{i-1}),x_i)$, where $\tau$ is a monotonic transformation of $x_i$ parameterised by $c_i$, e.g.~an affine transformation $T_i(x) = \alpha_i x_i + \beta_i$ where $c_i$ outputs $\alpha_i \neq 0$ and $\beta_i$. For instance, \cite{kingma} proposed \textit{inverse autoregressive flows} (IAF), taking $T(x) = \mu + \exp(\sigma) \odot x$.
Here $\odot$ is elementwise multiplication and $\mu$ and $\sigma$ are vectors output by an autoregressive neural network: one designed so that $\mu_i, \sigma_i$ depend on $x$ only through $x_j$ for $j<i$. In \cite{huang2018neural}, $\tau$ was the output of a monotonic neural network and the resulting flow was called a \textit{neural autoregressive flow} (NAF). Compositions of normalising flows can also be considered, of the form
\begin{equation}
T = T^{(n)} \circ \dots \circ T^{(1)}
\label{eq: NF compose}
\end{equation}
where each $T^{(i)}$ is itself a normalising flow e.g.~a IAF. For instance, \cite{dinh2014nice} proposed using \textit{coupling layers} of the form $T^{(i)}(x) = (h(x_1,\ldots,x_r),x_{r+1},\ldots,x_d)$, where $r < d$ and $h:\mathbb{R}^r\rightarrow\mathbb{R}^r$ is a bijection. These only update the first $r$ components of $x$, so they are typically composed with permutations.

Regardless of the provenance of a transport map $T$, all free parameters of $T$ are collectively denoted $\theta$, and are to be estimated. The suitability of a parametric set of candidate maps in combination with KSD is studied both empirically in \Cref{sec:experiments} and theoretically, next.


\section{Theoretical Assessment} \label{sec: theory}

In \Cref{subsec: exist} we affirm basic conditions on $P$ and $Q$ for a transport map to exist. In \Cref{subsec: consistent} we establish sufficient conditions for the consistency of our method and in \Cref{subsec: validate} we consider a particular class of transport maps based on neural networks, to demonstrate how our conditions on the transport map can be explicitly validated.


\subsection{Existence of an $L^2$ Transport Map} \label{subsec: exist}

For a complete separable metric space $\mathcal{X}$, recall that the \emph{Wasserstein space} of order $p \geq 1$ is defined by taking some $x_0 \in \mathcal{X}$ and
\begin{equation*}
\mathcal{P}_p(\mathcal{X}) \coloneqq \textstyle \left\{P\in\mathcal{P}(\mathcal{X}) :  \int \text{dist}(x,x_0)^p\,\mathrm{d}P(x) < \infty \right\} ,
\end{equation*}
where the definition is in fact independent of the choice of $x_0 \in \mathcal{X}$ \citep[][Definition 6.4]{villani_2009}.
For existence of a transport map, we make the following assumptions on $P$ and $Q$:

\begin{assumption}[Assumptions on $Q$] \label{assumption reference}
	The reference measure $Q\in\mathcal{P}(\mathcal{X})$, where $\mathcal{X}$ is a complete separable metric space, and $Q(\{x\}) = 0$ for all $x\in\mathcal{X}$.
\end{assumption}

\begin{assumption}[Assumptions on $P$] \label{assumption target}
	The target measure $P\in\mathcal{P}_2(\mathbb{R}^d)$ has a strictly positive density $p$ on $\mathbb{R}^d$. 
\end{assumption}

These assumptions guarantee the existence of a transport map with $L^2$ regularity, as shown in the following result:

\begin{proposition} \label{prop: transport map properties}
	If \Cref{assumption reference,assumption target} hold, then there exists a transport map $T \in \prod_{i=1}^d L^2(Q)$ such that $T_\# Q = P$.
\end{proposition}

Of course, such a transport map will not be unique in general.




\subsection{Consistent Posterior Approximation} \label{subsec: consistent}

The setting for our theoretical analysis considers a sequence $(\mathcal{T}_n)_{n \in \mathbb{N}}$ of parametric classes of transport map, where intuitively $\mathcal{T}_n$ provides a more flexible class of map as $n$ is increased.
For example, $\mathcal{T}_n$ could represent the class of triangular maps comprising of $n$th order polynomials, or a class of normalising flows comprising of $n$ layers in \eqref{eq: NF compose}.


\begin{assumption}[Assumptions on $\mathcal{T}_n$] \label{assum: G contains T}
	There exists a subset $\textgoth{T} \subseteq \prod_{i=1}^d L^2(Q)$ containing an element $T\in\textgoth{T}$ for which $T_\# Q=P$.
	The sequence $(\mathcal{T}_n)_{n \in \mathbb{N}}$ satisfies $\mathcal{T}_n \subseteq \textgoth{T}$ with $\mathcal{T}_n\subseteq\mathcal{T}_m$ for $n \leq m$ and $\mathcal{T}_\infty := \lim_{n \rightarrow \infty} \mathcal{T}_n$ is a dense set in $\textgoth{T}$.
\end{assumption} 

\Cref{prop: transport map properties} provides sufficient conditions for the set $\textgoth{T}$ in \Cref{assum: G contains T} to exist; the additional content of \Cref{assum: G contains T} ensures that $\mathcal{T}_\infty$ is rich enough to consistently approximate an exact transport map, in principle at least.
Next, we state our consistency result:

\begin{theorem}\label{theorem: convergence theorem}
	Let \Cref{assumption reference,assumption target,assum: G contains T} hold.
	Further suppose that $P$ is distantly dissipative, with $\nabla \log p$ Lipschitz and $\E_{X\sim P}[\|\nabla \log p(X)\|^2] < \infty$. 
	Suppose that $T_n \in \mathcal{T}_n$ satisfies
	\begin{equation}
	\mathcal{D}_{\textsc{S}}(P,(T_n)_\#Q) - \inf_{T\in\mathcal{T}_n} \mathcal{D}_{\textsc{S}}(P,T_\#Q) \stackrel{n\rightarrow \infty}{\rightarrow} 0 , \label{eq: main result}
	\end{equation}
	with $\mathcal{D}_{\textsc{S}}$ defined  in \Cref{theorem:gorham inverse multi quadric}.
	Then $(T_n)_\#Q \Rightarrow P$.
\end{theorem}

The statement in \eqref{eq: main result} accommodates the reality that, although finding the global optimum $T \in \mathcal{T}_n$ will typically be impractical, one can realistically expect to find an element $T_n$ that achieves an almost-as-low value of KSD, e.g. using a stochastic optimisation method.
To our knowledge, no comparable consistency guarantees exist for measure transport using KLD.


\subsection{Validating our Assumptions on $\mathcal{T}_n$} \label{subsec: validate}

Recall that earlier work on measure transport placed strong restrictions on the set of maps $\mathcal{T}_n$, requiring each map to be a diffeomorphism with non-vanishing Jacobian determinant.
In contrast, our assumptions on $\mathcal{T}_n$ are almost trivial; we do not require smoothness and there is not a bijection requirement.
Our assumptions can be satisfied \emph{in principle} whenever $\mathcal{X}$ is a complete separable metric space, since then $\prod_{i=1}^d L^2(Q)$ is separable \citep[][Proposition 3.4.5]{cohn2013measure} and admits a Schauder basis $\{\phi_i\}_{i \in \mathbb{N}}$, so we may take $\mathcal{T}_n = \text{span}\{\phi_1,\dots,\phi_n\}$ for \Cref{assum: G contains T} to hold. 
In practice we are able to verify \Cref{assum: G contains T} for quite non-trivial classes of map $\mathcal{T}_n$.
To demonstrate, one such example is presented next:

We consider deep neural networks with multi-layer perceptron architecture and ReLU activation functions
Let $\mathcal{R}_{l,n}(\mathbb{R}^p\rightarrow\mathbb{R}^d)$ denote the set of such \emph{ReLU neural networks} $f : \mathbb{R}^p \rightarrow \mathbb{R}^d$ with $l$ layers and width at most $n$. See \Cref{def: DNN} in \Cref{app: DNN} for a formal definition.

\begin{proposition} \label{prop: ReLU DNN}
	Let \Cref{assumption reference,assumption target} hold.
	Let $Q$ admit a positive, continuous and bounded density on $\mathcal{X} = \mathbb{R}^p$.
	Let $\mathcal{T}_n = \mathcal{R}_{l,n}(\mathbb{R}^p\rightarrow\mathbb{R}^d)$ with $l := \lceil \log_2(p+1) \rceil$. 
	Then \Cref{assum: G contains T} holds.
\end{proposition}

The maps in \Cref{prop: ReLU DNN} are not bijections, illustrating the greater flexibility of KSD compared to KLD for measure transport.
This completes our theoretical discussion, and our attention now turns to empirical assessment.



\section{Empirical Assessment} \label{sec:experiments}

The purpose of this section is to investigate whether KSD is competitive with KLD for measure transport. 
\Cref{subsec: toy examples} compares both approaches using a variety of transport maps and a synthetic test-bed. 
Then, in \Cref{subsec: biochemical oxygen,subsec: lotka-volterra} we consider more realistic posterior approximation problems arising from, respectively, a biochemical oxygen model and a parametric differential equation model.

In all experiments we used the kernel \eqref{eq: IMQ} with $c=1$, $\ell = 0.1$, $\beta = -1/2$ (other choices were investigated in \Cref{subsec: misspecified lengthscale}), the stochastic optimiser Adam with batch size $n=100$ and learning rate $0.001$ (other choices were investigated in \Cref{subsec: stochastic optimisation}), and the reference distribution $Q$ was taken to be a standard Gaussian on $\mathbb{R}^p$ (other choices were considered in \Cref{subsec: other Q}).
Code to reproduce these results is available at \url{https://github.com/MatthewAlexanderFisher/MTKSD}.


\subsection{Synthetic Test-Bed} \label{subsec: toy examples}

\begin{figure*}[t!] 
	\centering
	% high resolution version (slower to render)
	\includegraphics[width=1.\textwidth]{figures/main_fig.pdf}
	
	%low resolution version (quicker to render)
	%\includegraphics[width=1.\textwidth]{low_res_figures/low_res_main_fig.png} 
	\caption{
		Measure transport with KSD, versus KLD and HMC.
		The top row reports results for approximation of a sinusoidal density using an inverse autoregressive flow, while the bottom row reports analogous results for a multimodal density and a neural autoregressive flow. 
		The first three columns display convergence of the KSD-based method as the number of iterations of stochastic optimisation is increased.
		The remaining columns compare the output of the KLD-based method and HMC for an identical computational budget.
		% remember to change to full resolution plot
	}
	\label{fig: toy densities}
\end{figure*}


First we consider a set of synthetic examples that have previously been used to motivate measure transport as an alternative to MCMC.
Three targets were considered; $p_1$ is a sinusoidal density, $p_2$ is a banana density and $p_3$ is multimodal; these are formally defined in \Cref{subsec: details of toy models}. 
Results for $p_1$ and $p_3$ are displayed in \Cref{fig: toy densities}. 
The convergence of the approximation to the target is shown for KSD and the corresponding approximation after $10^4$ iterations of Adam is shown for KLD.
Since, for both objectives, one iteration requires $10^2$ evaluations of $\log p_i$ or its gradient, this represents a total of $10^6$ calls to $\log p_i$ or its gradient.
The corresponding approximation produced using an adaptive Hamiltonian Monte Carlo (HMC) algorithm \citep{hoffman2014no,betancourt2017conceptual} is shown, where the HMC chains were terminated once $10^6$ evaluations of $\log p_i$ or its gradient had been performed. 
%\chris{Could Matt please recommend a reference for HMC?}
Both $p_1$ and $p_3$ present challenges for HMC that, to some extent, can be overcome using measure transport.

The results in \Cref{fig: toy densities} are for a fixed class of transport map, but now we report a systematic comparison of KSD and KLD.
The majority of maps that we consider are diffeomorphic (in order that KLD can be used), implemented in Pyro \citep{bingham2018pyro}.
Since KSD does not place such requirements on the transport map, we also report results for a (non-bijective) ReLU neural network.
Our performance measure is an estimate of the Wasserstein-1 distance between the target and approximate distributions computed using $10^4$ samples (see \Cref{subsec: performance metrics} for details). Results are detailed in \Cref{table: toy density results}. Overall, there is no clear sense in which KSD out-performs KLD or \textit{vice versa}; KSD performed best on $p_1$, KLD performed best on $p_2$, and for $p_3$ the results were mixed. We conclude that these objectives offer similar performance for measure transport. However, KLD cannot be applied to the ReLU neural network (denoted N/A in \Cref{table: toy density results}) due to the strong constraints on the mapping that are required by KLD. 
\begin{table*}[t!] 
	\input{figures/results_table}
	\caption{Results from the synthetic test-bed. 
		The first column indicates which parametric class of transport map was used; full details for each class can be found in \Cref{subsec: details of toy models}.
		A map-dependent number of iterations of stochastic optimisation, $N$, are reported - this is to ensure that all optimisers approximately converged. 
		The main table reports the (first) Wasserstein distance between the approximation $T_\#Q$ and the target $P$. 
		Bold values indicate which of KSD or KLD performed best.
	}
	\label{table: toy density results}
\end{table*}

Two discussion points are now highlighted:
First, it is known that certain normalising flows can capture multiple modes due to their flexibility, however others cannot \citep{huang2018neural}. One solution is to consider a mixture of transport maps; i.e. $\sum_{i=1}^dw_i T^{(i)}_\# Q_i$ with reference distribution $Q_1 \times \dots \times Q_d$ and mixing weights $w_i>0$ satisfying $\sum_i w_i = 1$. This idea has been explored recently in \cite{pires2020variational}. In \Cref{table: toy density results} we report results using mixtures of \textit{inverse autoregressive flows} (IAF). As one might hope, these approximations were successful in finding each of the modes in $p_3$, but fared relatively worse for $p_1$ and $p_2$. Second, since in Adam we are using a Monte Carlo estimator of the gradient, it is natural to ask whether a quasi Monte Carlo estimator would offer an improvement \citep{wenzel2018quasi}. This was investigated and our results are reported in \Cref{subsec: QMC investigation}.





\subsection{Biochemical Oxygen Demand Model} \label{subsec: biochemical oxygen}

Next we reproduce an experiment that was used to illustrate measure transport using KLD in \cite{parno2018transport}. 
The task is parameter inference in a $d=2$ dimensional oxygen demand model, of the form $B(t) = \alpha_1(1 - \exp( - \alpha_2 t))$, where $B(t)$ is the biochemical oxygen demand at time $t$, a measure of the consumption of oxygen in a given water column sample due to the decay of organic matter \citep{sullivan2010biochemical}. The parameters to be inferred are $\alpha_1 , \alpha_2 > 0$. Full details of the prior and the likelihood are contained in \Cref{subsec: details of biochemical model}. 

For our experiment, we trained a \textit{block neural autoregressive flow}\footnote{This class of transport map was experimentally observed to outperform the other classes we considered.} using $N = 30,000$ iterations of Adam. Results are presented in \Cref{fig: bod results}. Unlike the synthetic experiments, we no longer have a closed form for the target $P$; however, this problem was amenable to MCMC and a long run of HMC ($10^6$ iterations, thinned by a factor of 100) provided a gold standard, allowing us to approximate the Wasserstein-1 distance from $T_\#Q$ to $P$ as in \Cref{subsec: toy examples}. For the KSD-based method, we obtained a Wasserstein-1 distance of $0.069$, while KLD achieved $0.015$. Although the Wasserstein-1 distance for KSD is larger than that for KLD, both values are close to the \textit{noise floor} for our approximation of the Wasserstein-1 distance; two independent runs of HMC ($10^6$ iterations, thinned by a factor of 100), differed in Wasserstein-1 distance by 0.022.
We therefore conclude that KSD and KLD performed comparably on this task.

\begin{figure*}[h!] 
	\centering
	\includegraphics[width=0.9\textwidth]{figures/bod_result.pdf} 
	\caption{
		Results for the biochemical oxygen demand model. 
		The leftmost panel is the target distribution, while the central and rightmost panels show samples generated from the output of the methods based, respectively, on KSD and KLD.
		% remember to change to full resolution plot
	}
	\label{fig: bod results}
\end{figure*}

\subsection{Generalised Lotka-Volterra Model} \label{subsec: lotka-volterra}

Our final experiment is a realistic inference problems involving a non-trivial likelihood. 
Following \cite{parno2018transport}, we consider parameter inference for a generalised Lotka--Volterra model
\begin{align}
\label{eq: LV}
\begin{split}
\textstyle \frac{\mathrm{d}p}{\mathrm{d}t}(t) &= \textstyle rp(t)\big(1 - \frac{p(t)}{k}\big) - s\frac{p(t)q(t)}{a + p(t)} , \\
\textstyle \frac{\mathrm{d}q}{\mathrm{d}t}(t) &= \textstyle u\frac{p(t)q(t)}{a + p(t)} - vq(t), 
\end{split}
\end{align}
where $p(t),q(t) > 0$ are the predator and prey populations respectively at time $t$ and $r, k, s, u, a$ and $v$, along with the initial conditions $p(0) = p_0$ and $q(0) = q_0$, are parameters to be inferred. 
Together, these $d=8$ parameters were inferred from a noisy dataset, with the prior and likelihood reported in \Cref{subsec: details of lotka volterra}.
This task is realistic and yet amenable to MCMC; the latter is an essential requirement to allow us to provide a gold standard against which to assess KSD and KLD, and we again used an extended run of HMC.

For this experiment, the B-NAF class and $N = 5 \cdot 10^4$ iterations of Adam were used.
The gradients, required both for HMC and KSD measure transport, were computed using automatic differentiation through the numerical integrator used to solve \eqref{eq: LV}, implemented in the \texttt{torchdiffeq} Python package \citep{chen2018neural}.

For the KSD-based method, we obtained an approximate Wasserstein-1 distance from $T_\#Q$ to $P$ of $0.130$, while KLD achieved $0.110$.
The noise floor for our approximation of the Wasserstein-1 distance in this case was $0.107$. 
We therefore conclude that KSD and KLD also performed comparably on this more challenging task.

\section{Discussion} \label{sec: discuss}

This paper proposed and studied measure transport using KSD, which can be seen as an instance of \emph{operator variational inference} \citep{ranganath2016operator}.
Our findings suggest that KSD is a suitable variational objective for measure transport; we observed empirical performance comparable with that of KLD, yet only minimal and verifiable conditions on the map $T$ were required.

There are three potential limitations of KSD compared to KLD: First, the parameters of the kernel must be specified, and a poor choice of kernel parameters can result in poor approximation; see \Cref{subsec: misspecified lengthscale}. It would be interesting to explore whether adversarial maximisation of KSD with respect to the kernel parameters, while minimising KSD over the choice of transport map, offers a solution \citep{grathwohl2020learning}. Second, while only first order derivatives are required for KLD, gradient-based optimisation of KSD requires second order derivatives of $p$. In most automatic differentiation frameworks, and for most models, this is possible at little extra computational cost, but sometimes this will present difficulties e.g. for models with differential equations involved. Third, it is known that score-based variational objectives can sometimes exhibit pathologies \citep{wenliang2020blindness}; some of these are illustrated in \Cref{subsec: pathologies}.

Several recent works explored the possibility of combining measure transport with Monte Carlo \citep{salimans2015markov,wolf2016variational,hoffman2017learning,caterini2018hamiltonian,prangle2019distilling,thin2020metflow} and it would also be interesting to consider the use of KSD in that context. Related, for both KSD and KLD there is freedom to select the space $\mathcal{X}$ and the reference distribution $Q$. This could also be handled within the optimisation framework, but further work would be needed to determine how these additional degrees of freedom should be parametrised.







==> Measure Transport with Kernel Stein Discrepancy/figures/different_reference_table.tex <==
\newcolumntype{Y}{>{\centering\arraybackslash}X} 


\begin{tabularx}{\textwidth}{@{}lYYY@{}} \toprule
     {Reference Distribution $Q$} & {Sinusoidal} & {Banana} & {Multimodal}  \\ \midrule
     Laplace         & $0.45$  & $0.25$ & $1.4$  \\ 
     Gaussian Mixture          & \textbf{$0.23$}  & $0.25$ & \textbf{$0.46$}  \\
     Gaussian & $0.38$ & \textbf{$0.20$} & $0.67$ \\ \bottomrule
\end{tabularx}


==> Measure Transport with Kernel Stein Discrepancy/figures/ksd_UvsV_table.tex <==
\newcolumntype{Y}{>{\centering\arraybackslash}X} 


\begin{tabularx}{\textwidth}{@{}llYYYYYY@{}} \toprule
        &  & \multicolumn{2}{c}{Sinusoidal}  & \multicolumn{2}{c}{Banana} & \multicolumn{2}{c}{Multimodal} \\
      \cmidrule(lr){3-4} \cmidrule(l){5-6} \cmidrule(l){7-8} 
     {Transport Map} & {$N$} & {KSD-U} & {KSD-V} & {KSD-U} & {KSD-V} &  {KSD-U} & {KSD-V} \\ \midrule
     IAF  & $10^4$                & $\textbf{0.38}$  & $0.39$ & $\bf{0.20}$ & 0.25  & 0.67 & $\bf{0.61}$ \\
     IAF (stable) & $10^4$        & $\textbf{0.35}$ & 0.36 & $\bf{0.16}$  &  0.19 & \textbf{0.61}  & $\bf{0.61}$ \\ 
     NAF   & $10^4$               & $\textbf{0.55}$ & 0.58  & $\bf{0.39}$  & 0.43 &  \textbf{0.095} & 0.12  \\ 
     SAF  & $10^4$                & $\textbf{0.23}$ & 0.27  & $\bf{0.20}$  & 0.48 & \textbf{0.30}  & 1.2 \\ 
     B-NAF  & $10^4$                & $\textbf{0.78}$ & 0.85  & $\bf{0.70}$  & $\bf{0.70}$ & $\bf{1.0}$   & $\bf{1.0}$  \\ 
     Polynomial (cubic)  & $10^4$ & $\textbf{0.40}$ & 0.61 & $\bf{0.25}$  & $0.41$ & 0.51  & $\bf{0.40}$ \\ 
    IAF mixture  & $3{\times}10^4$ & $\bf{1.3}$ & $\bf{1.3}$ & $\bf{0.19}$  & 0.39  & $\bf{0.037}$  & 0.040 \\ 
     ReLU network & $5{\times} 10^4$& $\textbf{0.71}$ & 0.96 & \textbf{0.43}  & 0.53  & \textbf{0.22}  &  1.2 \\\bottomrule
\end{tabularx}


==> Measure Transport with Kernel Stein Discrepancy/figures/optimisation_table.tex <==
\newcolumntype{Y}{>{\centering\arraybackslash}X} 


\begin{tabularx}{\textwidth}{@{}lYYYY@{}} \toprule
          & \multicolumn{4}{c}{Batch size}  \\
      \cmidrule(lr){2-5}
     {Optimisation method} & {$25$} & {$50$} & {$100$} & {$200$} \\ \midrule
     Adam ($l = 0.001$)          & $0.594$  & $0.546$ & $0.121$ & $\bf{0.0827}$ \\
     Adam ($l = 0.01$)       & $0.663$ & $0.768$ & $0.726$  & $\bf{0.242}$ \\ \midrule
     Adagrad ($l = 0.001$)              & $0.630$ & $0.620$ & $0.617$  & $\bf{0.616}$ \\ 
     Adagrad ($l = 0.01$)                  & $0.612$ & $0.608$ & $0.606$  & $0.602$ \\  \midrule
     RMSprop ($l = 0.001$)              & $0.590$ & $0.504$ & $0.144$  & $\bf{0.0856}$ \\ 
     RMSprop ($l = 0.01$)                  & $1.00$ & $0.699$ & $\bf{0.0653}$ & $0.125$ \\  \midrule
     SGD ($l = 0.001$)              & $0.902$ & $\bf{0.194}$ & $0.402$  & $0.433$ \\ 
     SGD ($l = 0.005$)                  & $1.24$ & $0.265$ & $\bf{0.143}$  & $0.241$  \\  \midrule
     ASGD ($l = 0.001$)              & $0.701$ & $\bf{0.34}$ & $0.401$  & $0.432$ \\ 
     ASGD ($l = 0.005$)                  & N/A & $\bf{0.166}$ & $0.478$  & $0.391$\\  \bottomrule
\end{tabularx}


==> Measure Transport with Kernel Stein Discrepancy/figures/qmc_table.tex <==
\newcolumntype{Y}{>{\centering\arraybackslash}X} 



\begin{tabularx}{\textwidth}{@{}lYYY@{}} \toprule
     {Sampling Method} & {Sinusoidal} & {Banana} & {Multimodal}  \\ \midrule
     Random shifted (modulo 1) grid       & $0.59$  & $0.53$ & $0.22$  \\ 
     Monte Carlo      & $\bf{0.55}$  & $\bf{0.39}$ & $\bf{0.16}$  \\ \bottomrule
\end{tabularx}


==> Measure Transport with Kernel Stein Discrepancy/figures/relu_dimension_table.tex <==
\newcolumntype{Y}{>{\centering\arraybackslash}X} 


\begin{tabularx}{\textwidth}{@{}lYYYYY@{}} \toprule
     Input dimension & {$p=1$} & {$p=2$} & {$p=3$} & {$p=4$} & $p=5$  \\ \midrule
     $W_1$ & $0.88$ & $0.39$ & $0.19$ & $0.27$ & $0.31$ \\ \bottomrule
\end{tabularx}


==> Measure Transport with Kernel Stein Discrepancy/figures/results_table.tex <==
\newcolumntype{Y}{>{\raggedright\arraybackslash}X} 


\begin{tabularx}{\textwidth}{@{}llYYYYYY@{}} \toprule
        &  & \multicolumn{2}{c}{Sinusoidal}  & \multicolumn{2}{c}{Banana} & \multicolumn{2}{c}{Multimodal} \\
      \cmidrule(lr){3-4} \cmidrule(l){5-6} \cmidrule(l){7-8} 
     {Transport Map} & {$N$} & {KSD} & {KLD} & {KSD} & {KLD} &  {KSD} & {KLD} \\ \midrule
     IAF  & $10^4$                & $\textbf{0.38}$  & $0.52$ & 0.20 & \textbf{0.07}  & \textbf{0.67} & 1.1 \\
     IAF (stable) & $10^4$        & $\textbf{0.35}$ & $0.39$ & 0.16  & \textbf{0.11} & \textbf{0.61}  & 0.62 \\ 
     NAF   & $10^4$               & $\textbf{0.55}$ & $0.64$ & 0.39  & \textbf{0.025} &  \textbf{0.095} & 0.11 \\ 
     SAF  & $10^4$                & $\textbf{0.23}$ & $0.58$ & 0.20  & \textbf{0.18} & \textbf{0.30}  & 0.48 \\ 
     B-NAF  & $10^4$                & $\textbf{0.78}$ & $1.2$ & 0.70  & \textbf{0.18} & 1.0   & \textbf{0.99}  \\ 
     Polynomial (cubic)  & $10^4$ & $\textbf{0.40}$ & $0.84$ & 0.25  & \textbf{0.059} & 0.51  & \textbf{0.43} \\ 
     IAF mixture  & $3{\times}10^4$        & $1.29$ & $\textbf{0.61}$ & 0.19  & \textbf{0.14} & 0.037  & \textbf{0.036} \\ 
     ReLU network & $5{\times} 10^4$        & $\textbf{0.71}$ & N/A & \textbf{0.43}  & N/A & \textbf{0.22}  & N/A \\\bottomrule
\end{tabularx}

